Countering the Over-Reliance Trap: Mitigating Object Hallucination for LVLMs via a Self-Validation Framework

Despite progress in Large Vision Language Models (LVLMs), object hallucination remains a critical issue in image captioning task, where models generate descriptions of non-existent objects, compromising their reliability. Previous work attributes this to LVLMs' over-reliance on language priors and attempts to mitigate it through logits calibration. However, they still lack a thorough analysis of the over-reliance. To gain a deeper understanding of over-reliance, we conduct a series of preliminary experiments, indicating that as the generation length increases, LVLMs' over-reliance on language priors leads to inflated probability of hallucinated object tokens, consequently exacerbating object hallucination. To circumvent this issue, we propose Language-Prior-Free Verification to enable LVLMs to faithfully verify the confidence of object existence. Based on this, we propose a novel training-free Self-Validation Framework to counter the over-reliance trap. It first validates objects' existence in sampled candidate captions and further mitigates object hallucination via caption selection or aggregation. Experiment results demonstrate that our framework mitigates object hallucination significantly in image captioning task (e.g., 65.6% improvement on CHAIRI metric with LLaVA-v1.5-7B), surpassing the previous SOTA methods. This result highlights a novel path towards mitigating hallucination by unlocking the inherent potential within LVLMs themselves.

==> figures/finding1.tex <==
\begin{figure}[t] % 子图宽度占主文本宽度的48%
    \centering
    \includegraphics[width=1.0\linewidth]{figures/bin.pdf} % 插入图片1
    \caption{
    JSD of object position 
    % Low discrepancy indicates an over-reliance of textual information.
    } % 子图标题
    \label{fig:sub1} % 子图标签（可用于交叉引用）
\end{figure}

==> figures/first-case.tex <==
\definecolor{forestgreen}{RGB}{0, 176, 80}
\begin{figure}[t] % 子图宽度占主文本宽度的48%
    \centering
    \includegraphics[width=1.0\linewidth]{figures/case1.png} % 插入图片1
    \caption{
% An example of self-validating. 
Hallucinated objects are highlighted in \textcolor{red}{red} while existent objects are in \textcolor{forestgreen}{green}. The LVLM provides a more discriminative existence estimation of the objects when answering in one word, indicating that LVLM has the ability to self-validate the objects in generated caption.
% shows different logical consistency to hallucinated object “apple” and existent object “banana”.
% The one-word brief answer provides a more discriminative estimation of the existence of objects by avoiding reliance on generated text.
% 这张图indicate 利用answer-briefly策略，LVLM有能力去自我验证生成的objects
    } % 子图标题
    \label{fig:first} % 子图标签（可用于交叉引用）
\end{figure}

==> tables/gpt-score.tex <==
\begin{table}[t]
  \centering
  % \small
    \setlength{\tabcolsep}{5pt}
    \begin{tabular}{llcc}
    \toprule
    Model & Method & Acc. & Rel. \\
    \midrule
    \multirow{3}{*}{LLaVA-1.5 \scriptsize{(7b)}} & - & 7.04 & 7.29 \\
    & \textbf{Ours~\scriptsize{(w/BoN.)}} & \textbf{7.47} & \textbf{7.98} \\
    & \textbf{Ours~\scriptsize{(w/FtA.)}} & 7.39 & 7.76 \\
    \midrule
    \multirow{3}{*}{LLaVA-1.5 \scriptsize{(13b)}} & - & 7.65 & 7.95 \\
    & \textbf{Ours~\scriptsize{(w/BoN.)}} & 7.72 & 8.20 \\
    & \textbf{Ours~\scriptsize{(w/FtA.)}} & \textbf{7.96} & \textbf{8.32} \\
    \midrule
    \multirow{3}{*}{mPLUG-Owl2 \scriptsize{(7b)}} & - & 7.28 & 7.66 \\
    & \textbf{Ours~\scriptsize{(w/BoN.)}} & \textbf{7.38} & \textbf{7.96} \\
    & \textbf{Ours~\scriptsize{(w/FtA.)}} & 7.22 & 7.76 \\

    
    \bottomrule
    \end{tabular}
  \caption{GPT-assisted evaluation. Acc. indicates Accuracy, while Rel. indicates Relevancy.}
  \label{tab:gpt-results}
\end{table}%
